Once Detected, Never Lost: Surpassing Human Performance in Offline LiDAR based 3D Object Detection

This paper aims for high-performance offline LiDAR-based 3D object detection. We first observe that experienced human annotators annotate objects from a track-centric perspective. They first label the objects with clear shapes in a track, and then leverage the temporal coherence to infer the annotations of obscure objects. Drawing inspiration from this, we propose a high-performance offline detector in a track-centric perspective instead of the conventional object-centric perspective. Our method features a bidirectional tracking module and a track-centric learning module. Such a design allows our detector to infer and refine a complete track once the object is detected at a certain moment. We refer to this characteristic as "onCe detecTed, neveR Lost" and name the proposed system CTRL. Extensive experiments demonstrate the remarkable performance of our method, surpassing the human-level annotating accuracy and the previous state-of-the-art methods in the highly competitive Waymo Open Dataset without model ensemble. The code will be made publicly available at https://github.com/tusen-ai/SST.

==> experiments/robust.tex <==
Our framework takes the full-length tracks as input, so it could be a major concern if the results are sensitive to tracking results.
To answer the question, we add two kinds of noise to the input tracks.
\begin{itemize}
    \item We randomly split input tracks into two parts to mimic the to early termination in tracking.
    \item We randomly swap two parts on two tracks to mimic the wrong association in tracking.
\end{itemize}
Table~\ref{tab:tracking_noise} shows the results.
\input{tables/tracking_noise}

==> tables/assign.tex <==

% \begin{table}[h]
% 	\begin{center}
% 		\resizebox{0.99\columnwidth}{!}{
% 			\begin{tabular}{l|ccc|c}
% 				\toprule
			
% 				\multirow{2}{*}{Techniques} &\multicolumn{3}{c}{L2 3D AP/APH}  \\
% 				 & Vehicle & Pedestrian & Cyclist \\
% 				\midrule
% 				Single-frame FSD            \\
%                     Multi-frame FSD            \\
% 				Offline FSD  \\
% 				Track Refinement  \\
%     			Bidirection  \\
%     			Track TTA  \\
% 				 \bottomrule
% 			\end{tabular}
% 		}	
% 	\end{center}
% 		\caption{hh}
% \end{table}

==> tables/failure_cases_bfn.tex <==
\begin{table}[h]
	\small
	\begin{center}
		\resizebox{0.9\columnwidth}{!}{
			\begin{tabular}{l|cc|cc}
				\toprule
				& 			
				\multicolumn{2}{c|}{\emph{Vehicle} } & \multicolumn{2}{c}{\emph{Pedestrian} } \\
				& Base  & Refined & Base & Refined \\
				\midrule
				BFN ratio   \\
                    \#points \\
                    Avg. velo. \\
                    AP   \\
				 \bottomrule
			\end{tabular}
		}	
	\end{center}
	\caption{hh}
	\label{tab:BFN}
\end{table}

==> tables/failure_cases_hfp.tex <==
\begin{table}[h]
	\small
	\begin{center}
		\resizebox{0.95\columnwidth}{!}{
			\begin{tabular}{l|cc|cc}
				\toprule
				& 			
				\multicolumn{2}{c|}{\emph{Vehicle} ($s_t$ = xx)} & \multicolumn{2}{c}{\emph{Pedestrian} ($s_t$ = xx)} \\
				& Base  & Refined & Base & Refined \\
				\midrule
				HFP ratio   \\
                    Original AP   \\
                    Corrected AP   \\
				 \bottomrule
			\end{tabular}
		}	
	\end{center}
	\caption{hh}
	\label{tab:HFP}
\end{table}

==> tables/human_bfn.tex <==
\begin{table}[h]
	\begin{center}
		\resizebox{0.99\columnwidth}{!}{
			\begin{tabular}{l|cccc}
				\toprule
			
				\multirow{2}{*}{\shortstack[1]{Result \\ source }} &\multicolumn{4}{c}{Vehicle 3D AP with different IoUs}  \\
				& IoU=0.6 & IoU=0.5 & IoU=0.4 & IoU=0.3 \\
				\midrule
				Human  &76.05/74.67& 72.23/71.77 & 76.83/74.02 & 79.08/78.21 \\
				Ours  &76.03/74.66& 72.20/71.75 & 76.88/74.07 & 79.00/78.15 \\

				 \bottomrule
			\end{tabular}
		}	
	\end{center}
		\caption{hh}
	\label{tab:human_bfn}
\end{table}

==> tables/misc_back.tex <==
\begin{table*}[t]
\vspace{-.2em}
\centering
%#################################################
% MAE decoder depth
%#################################################
\subfloat[
\textbf{Track length}. 
\label{tab:decoder_depth}
]{
\centering
\begin{minipage}{0.29\linewidth}{\begin{center}
\tablestyle{4pt}{1.05}
% \begin{tabular}{x{18}x{24}x{24}}
\begin{tabular}{c|cc}
Lengths & Veh. & Ped. \\
 \hline
10 & 84.8 & 65.5 \\
20 & \textbf{84.9} & 70.0 \\
50 & \textbf{84.9} & 71.9 \\
100 &  {\textbf{84.9}} &  {\textbf{73.5}} \\
200 & 84.4 & 73.3 \\
\end{tabular}
\end{center}}\end{minipage}
}
\hspace{2em}
%#################################################
% MAE decoder width
%#################################################
\subfloat[
\textbf{Track TTA}.
\label{tab:decoder_width}
]{
\begin{minipage}{0.29\linewidth}{\begin{center}
\tablestyle{4pt}{1.05}
% \begin{tabular}{x{18}x{24}x{24}}
\begin{tabular}{ccc}
Strategy & ft & lin \\
 \hline
None & \textbf{84.9} & 69.1 \\
Rotation & 84.8 & 71.3 \\
Double Flip &  {\textbf{84.9}} &  {\textbf{73.5}} \\
All & 84.4 & 73.1 \\
\end{tabular}
\end{center}}\end{minipage}
}
\hspace{2em}
%#################################################
% MAE with mask token on encoder
%#################################################
\subfloat[
\textbf{Separating motion states}.
\label{tab:mask_token}
]{
\begin{minipage}{0.29\linewidth}{\begin{center}
\tablestyle{4pt}{1.2}
% \begin{tabular}{y{56}x{24}x{24}z{24}}
\begin{tabular}{c|cc}
case & Veh. & Ped.  \\
 \hline
Separating & 84.2 & 59.6 $\times$ \\
Merging &  {\textbf{84.9}} &  {\textbf{73.5}}  \\
\multicolumn{3}{c}{~}\\
\multicolumn{3}{c}{~}\\
% \multicolumn{3}{c}{~}\\
\end{tabular}
\end{center}}\end{minipage}
}
\\
\centering
\vspace{.3em}
%#################################################
% MAE targets
%#################################################
\subfloat[
\textbf{The number of frames in the base detector.}. 
\label{tab:mae_target} are effective.
]{
\begin{minipage}{0.29\linewidth}{\begin{center}
\tablestyle{6pt}{1.05}
% \begin{tabular}{y{54}x{24}x{24}}
\begin{tabular}{ccc}
Frames & Veh. & Ped. \\
 \hline
$[-4, 0]$  &  {84.9} &  {73.5} \\
$[-4, 4]$ & \textbf{85.4} & \textbf{73.9} \\
$[-8, 8, \text{::}2]$ & 84.6 & 72.3 \\
$[-8, 8, \text{::}2]$ + framedrop & 85.3 & 71.6 \\
\end{tabular}
\end{center}}\end{minipage}
}
\hspace{2em}
%#################################################
% MAE data aug
%#################################################
\subfloat[
\textbf{Data augmentation}. Our MAE works with minimal or no augmentation.
\label{tab:aug}
]{
\centering
\begin{minipage}{0.29\linewidth}{\begin{center}
\tablestyle{4pt}{1.05}
% \begin{tabular}{y{54}x{22}x{22}}
\begin{tabular}{ccc}
case & ft & lin \\
 \hline
none & 84.0 & 65.7 \\
crop, fixed size & 84.7 & 73.1 \\
crop, rand size &  {\textbf{84.9}} &  {\textbf{73.5}} \\
crop + color jit & 84.3 & 71.9 \\
\end{tabular}
\end{center}}
\end{minipage}
}
\hspace{2em}
%#################################################
% MAE with mask types
%#################################################
\subfloat[
\textbf{Mask sampling}.
\label{tab:mask_types}
]{
\begin{minipage}{0.29\linewidth}{\begin{center}
\tablestyle{1pt}{1.05}
% \begin{tabular}{y{28}x{24}x{24}x{24}}
\begin{tabular}{cccc}
case & ratio & ft & lin \\
 \hline
random & 75 &  {\textbf{84.9}} &  {\textbf{73.5}} \\
block & 50 & 83.9 & 72.3 \\
block & 75 & 82.8 & 63.9 \\
grid & 75 & 84.0 & 66.0 \\
\end{tabular}
\end{center}}\end{minipage}
}
%#################################################
\vspace{-.1em}
\caption{}
\label{tab:ablations} \vspace{-.5em}
\end{table*}
%##################################################################################################

==> tables/tracking_noise.tex <==
\begin{table}[h]
	\begin{center}
		\resizebox{0.9\columnwidth}{!}{
			\begin{tabular}{l|cccc}
				\toprule
			
				\multirow{2}{*}{\shortstack[1]{Breaking \\ Ratio} } &\multicolumn{4}{c}{L2 3D AP/APH}  \\
				& Mean & Vehicle & Pedestrian & Cyclist \\
				\midrule
				0\%            \\
				10\%  \\
				50\%  \\
    			100\% \\

				 \bottomrule
			\end{tabular}
		}	
	\end{center}
		\caption{hh}
	\label{tab:tracking_noise}
\end{table}

==> tables/waymo_test_small.tex <==
\begin{table}[ht]
\small
\centering
% \setlength{\tabcolsep}{2.4mm}{

\resizebox{0.99\linewidth}{!}{
\begin{tabular}{l|c|c|c|c}
  % \specialrule{1pt}{0pt}{1pt}
\toprule
% \multirow{2}{*}{Methods}  & \multirow{2}{*}{\shortstack[1]{mAPH\\ L2}} & \multicolumn{2}{c|}{\textit{Vehicle} 3D AP/APH} & \multicolumn{2}{c|}{\textit{Pedestrian} 3D AP/APH} & \multicolumn{2}{c}{\textit{Cyclist} 3D AP/APH}\\
Methods & L2 mAPH\dag &  Veh. L1       &   Ped. L1     &   Cyc. L1      \\
\midrule

\textbf{\name (Ours)} &  82.52 &   90.08   & 90.17       &     84.06        \\

HRI\_ADLAB\_HZ & 81.32 &  	86.77  & 88.59     &     85.67       \\

LoGoNet\_Ens\ddag & 81.02 &  	88.33 &   88.98      &     83.10        \\

MT-Net v2~\cite{mtnet} & 80.00 &     87.54 &  87.62&          82.80       \\

BEVFusion-TTA\ddag~\cite{bevfusion} & 79.97 &  	87.96 &  87.64&          82.53       \\

LidarMultiNet-TTA~\cite{lidarmutlinet} & 79.94 &  	87.64  & 87.75&         82.77       \\

MPPNetEns~\cite{mppnet}  & 79.60 &  	87.77 &  87.92&         80.74       \\
% 3DAM\_Ens  & 79.19 &  	87.31/86.85 & 80.78/80.34 & 87.55/84.42&     82.52/79.45&    80.97/80.07 &     78.65/77.77  \\

% LIVOX\_Detection  & 78.96 &  	86.81/86.45 & 80.41/80.05 & 87.17/84.57&     82.16/79.59&    80.46/79.59 &     78.08/77.24  \\

% MT3D  & 78.73 &  	86.77/86.39 & 79.84/79.47 & 86.92/84.10	&     81.38/78.63&    81.40/80.52 &     78.95/78.10  \\
\bottomrule
  % \specialrule{1pt}{1pt}{0pt}
\end{tabular}
% }
}
\caption{
    \textbf{Top-performing methods in the leaderboard of Waymo Open Dataset}.
    We do not adopt model ensemble.
    \dag: Official metric for ranking.
    \ddag: Multi-modal method.
    }
 \label{tab:wod_test}

\end{table}
